The area of horizons and the trapped region

This paper considers some fundamental questions concerning marginally trapped surfaces, or apparent horizons, in Cauchy data sets for the Einstein equation. An area estimate for outermost marginally trapped surfaces is proved. The proof makes use of an existence result for marginal surfaces, in the presence of barriers, curvature estimates, together with a novel surgery construction for marginal surfaces. These results are applied to characterize the boundary of the trapped region.

==> extern/draft_commands.tex <==
\usepackage{ifthen}

%% Collect Time and Date Info
\makeatletter
\newcommand{\pt@twodigit}[1]{{\pt@tmp=#1\relax\ifnum\pt@tmp<10 0\fi\the\pt@tmp}}
\newcount\pt@hours
\newcount\pt@minutes
\newcount\pt@tmp
\newcommand{\printtime}{%
\pt@hours=\time%
\divide\pt@hours by 60\relax%
\pt@tmp=\pt@hours%
\multiply\pt@tmp by -60\relax%
\pt@minutes=\time%
\advance\pt@minutes by \pt@tmp%
\pt@twodigit\pt@hours:\pt@twodigit\pt@minutes}

%% How to put Info in the margin
\newlength{\mt@MarginWidth}
\newlength{\mt@PageHeight}
\newlength{\mt@ActualWidth}
\newlength{\mt@MaxWidth}
\newlength{\mt@FontSize}
\newlength{\mt@RightSkip}
\newlength{\mt@TextHeight}
\newlength{\mt@OffsetX}
\newlength{\mt@OffsetY}

\usepackage{eso-pic}
\usepackage{type1cm}
\usepackage{graphicx}

\newcommand{\margintext}[1]{
  \ifx\pdfoutput\undefined\write16{WARNING: Margintext
      will only correctly show up in PS - FILE!}
  \fi
  \AddToShipoutPicture{%
    \setlength{\mt@MarginWidth}{\oddsidemargin}%
    \addtolength{\mt@MarginWidth}{1in}%
    \setlength{\mt@PageHeight}{\paperheight}%
    \setlength{\mt@MaxWidth}{.8\mt@MarginWidth}%
    \setlength{\mt@FontSize}{12mm}%
    \setlength{\mt@RightSkip}{3mm}%
    \setlength{\mt@ActualWidth}{15mm}%
    \ifthenelse{\lengthtest{\mt@ActualWidth > \mt@MaxWidth}}%
    {
      \setlength{\mt@FontSize}{.6\mt@MarginWidth}
      \setlength{\mt@RightSkip}{.2\mt@MarginWidth}
      \setlength{\mt@ActualWidth}{.8\mt@MarginWidth}
    }{}
    \setlength{\mt@OffsetX}{\mt@ActualWidth}
    \setlength{\mt@OffsetY}{0mm}
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\mt@OffsetX,\strip@pt\mt@OffsetY){%
      \rotatebox{90}
        {
          \makebox[\mt@PageHeight][c]
          {\textcolor[gray]{0.75}{\fontfamily{cmss}
              \fontseries{m}
              \fontshape{n}
              \fontsize{\mt@FontSize}{\mt@FontSize}
              \selectfont{#1}}}
        }
      }
    }
}

%% Collect information from Subversion
% If the file svn_version.tex exists, we will read it, in there
% the command \svnVersion is defined. If the file does not exist, we
% print a warning and set \svnVersion to Unknown
\newboolean{draftmargin}
\setboolean{draftmargin}{false}

\IfFileExists{draft_control.tex}{%
\message{Draft control file exists.}%
\input{draft_control.tex}%
}{% 
\message{ WARNING: draft_control.tex not found.}%
\newcommand{\svnVersion}{???}%
}


\ifthenelse{ \boolean{draftmargin} }
        {
                \margintext{Rev: {\svnVersion}\hspace{1em}Built: {\the\year-\pt@twodigit\month-\pt@twodigit\day} {\printtime}}
        }
        {}

\makeatother



==> extern/layout_commands.tex <==
\usepackage{ifthen}
\usepackage{amsmath}
\usepackage{amsthm}

\makeatletter

\newcommand{\titlefamily}{}%
\newcommand{\thmfamily}{}%
\newcommand{\sectitlefnt}{}%
\newcommand{\subsectitlefnt}{}%
\newcommand{\ps@footnumber}{}

%% Typesetting equations
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand{\fillbox}{\hspace*{\fill}\ensuremath{\Box}}
\renewcommand{\qedsymbol}{\fillbox}

\ifthenelse{\isundefined{\nofancylayout}}
{%
  \renewcommand{\titlefamily}{\sffamily}%
  \renewcommand{\thmfamily}{\sffamily}%
  \renewcommand{\sectitlefnt}{\titlefamily\bfseries\Large}%
  \renewcommand{\subsectitlefnt}{\titlefamily\bfseries}%
  % 
  %% Paper size and margins
  % \usepackage[shiftmargins]{vmargin}
  % \setpapersize{A4}%
  % \setmarginsrb{35mm}{25mm}{30mm}{25mm}{0mm}{0mm}{10mm}{3\baselineskip}%
  %
  \usepackage{calc}
  \usepackage[totalwidth=75ex,totalheight=41\baselineskip,vmarginratio=4:5,footskip=3\baselineskip,hcentering]{geometry}
  
  %% Typesetting the titles
  \renewcommand{\section}{\@startsection%
    {section}%
    {1}%
    {0mm}%
    {-\baselineskip}%
    {\baselineskip}%
    {\sectitlefnt}}%
  \renewcommand{\subsection}{\@startsection
    {subsection}%
    {2}%
    {0mm}%
    {-\baselineskip}%
    {0.5\baselineskip}%
    {\subsectitlefnt}}%
  \renewcommand{\ps@footnumber}{%
    \renewcommand{\@oddhead}{}%
    \renewcommand{\@evenhead}{}%
    \renewcommand{\@oddfoot}{\hfill{\thepage}}%
    \renewcommand{\@evenfoot}{{\thepage}\hfill}}
  \makeatother
  % 
  %% Typesetting Paragraphs
  \setlength{\parskip}{1ex plus .5ex minus 0ex}
  \setlength{\parindent}{0em}
  % 
  %% Typesetting Theorems
  \newtheoremstyle{my_plain}%
  {\parskip}% above skip
  {\parskip}% below skip
  {\normalfont\itshape}% body font
  {}% indent
  {\normalfont\thmfamily\bfseries}% head font
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  \newtheoremstyle{my_remark}%
  {\parskip}% aboveskip
  {\parskip}% belowskip
  {\normalfont}% bodyfont
  {}% indent
  {\normalfont\thmfamily\bfseries}% headfont
  {.}% headpunct
  { }% headspace
  {}% custom-head-spec
  
  {
    \theoremstyle{my_plain}
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{definition}[theorem]{Definition}
  }
  
  {
    \theoremstyle{my_remark}
    \newtheorem{remark}[theorem]{Remark}
  }
    
}{%
  \newtheorem{theorem}{Theorem}[section]%
  \newtheorem{proposition}[theorem]{Proposition}%
  \newtheorem{corollary}[theorem]{Corollary}%
  \newtheorem{lemma}[theorem]{Lemma}%
  \newtheorem{definition}[theorem]{Definition}%
  \theoremstyle{remark}%
  \newtheorem{remark}[theorem]{Remark}%
}

\newenvironment{abst}{\begin{quote}\small\thmfamily\bfseries
    Abstract. \normalfont\small}{\end{quote}}

